TEST-V: TEst-time Support-set Tuning for Zero-shot Video Classification

Recently, adapting Vision Language Models (VLMs) to zero-shot visual classification by tuning class embedding with a few prompts (Test-time Prompt Tuning, TPT) or replacing class names with generated visual samples (support-set) has shown promising results. However, TPT cannot avoid the semantic gap between modalities while the support-set cannot be tuned. To this end, we draw on each other's strengths and propose a novel framework namely TEst-time Support-set Tuning for zero-shot Video Classification (TEST-V). It first dilates the support-set with multiple prompts (Multi-prompting Support-set Dilation, MSD) and then erodes the support-set via learnable weights to mine key cues dynamically (Temporal-aware Support-set Erosion, TSE). Specifically, i) MSD expands the support samples for each class based on multiple prompts enquired from LLMs to enrich the diversity of the support-set. ii) TSE tunes the support-set with factorized learnable weights according to the temporal prediction consistency in a self-supervised manner to dig pivotal supporting cues for each class. $\textbf{TEST-V}$ achieves state-of-the-art results across four benchmarks and has good interpretability for the support-set dilation and erosion.

==> tabs/AB-MS_strategy.tex <==
\begin{table}[!h]
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
        \toprule[1pt]
         \textbf{Frame Sequence}      & \textbf{HMDB-51}      & \textbf{UCF-101} \\ 
        \hline
        6 , 8          & $52.1$              & $78.2$   \\
        4 , 6 , 8      & $\mathbf{52.5}$              & $\mathbf{78.4}$   \\
        2 , 4 , 6 , 8  & $51.8$              & $78.0$   \\
        \bottomrule[1pt]
    \end{tabular}
    \caption{Effect of different frame sequences in multi-scale strategies.}
    \label{tab::MSS}
\end{table}
